Quantization of Schr\"odinger-Virasoro Lie algebra

In this paper, we use the general quantization method by Drinfel'd twists to quantize the Schr\"odinger-Virasoro Lie algebra whose Lie bialgebra structures were recently discovered by Han-Li-Su. We give two different kinds of Drinfel'd twists, which are then used to construct the corresponding Hopf algebraic structrues. Our results extend the class of examples of noncommutative and noncocommutative Hopf algebras.

==> 0284087.tex <==
%auto-ignore
